An Enterprise Control Assessment Case Study of the Energy-Water Nexus for the ISO New England System

The electric power generation mix of ISO New England (ISO-NE) is fundamentally changing. Nuclear, coal, and oil generation facilities are retiring while natural gas, solar, and wind generation are being adopted to replace them. Variable renewable energy (VREs) such as solar and wind present multiple operational challenges that require new and innovative changes to how the electricity grid is managed and controlled. Within the context of a New England case study, this paper looks at ways in which the water supply systems (water and wastewater treatment), and water dependent electricity generating resources (hydro, and thermal power plants) can be operated flexibly to help balance energy in an evolving grid. The study's methodology employs the novel but now well published Electric Power Enterprise Control System (EPECS) simulator to study the electric power systems operation, and the System-Level Generic Model (SGEM) to study the associated water consumption and withdrawals. This work studies six potential 2040 scenarios for the energy-water nexus of the ISO-NE system. It presents a holistic analysis that quantifies power system imbalances, normal operating reserves, energy market production costs, and water withdrawal and consumption figures. For scenarios with a high penetration of VREs, the study shows great potential of water resources to enhance grid flexibility through the provision of load-following, ramping, and regulation reserves by water resources. The work also provides significant insights on how to jointly control the water and energy supply systems to aid in their synergistic integration.

==> images-results/2040dnLFRStatisticsDel.tex <==
\begin{footnotesize}
\begin{center}
\begin{tabular}{p{3.5cm}rrrrrr}\toprule
 & \textbf{2040-1}& \textbf{2040-2}& \textbf{2040-3}& \textbf{2040-4}& \textbf{2040-5}& \textbf{2040-6}\\\toprule
\textbf{Up LFR Mean} (MW)&   208 &   172 &    66 &   207 &   194 &    58 \\\midrule
\textbf{Up LFR STD} (MW) &     8 &   -56 &   -17 &   -42 &   -68 &   -36 \\\midrule
\textbf{Up LFR Max} (MW)&   178 &   228 &   335 &   243 &   108 &   687 \\\midrule
\textbf{Up LFR Min} (MW)&   212 &   311 &   -96 &   221 &   213 &   423 \\\midrule
\textbf{Up LFR 95 percentile$^1$} (MW)&   241 &   283 &     6 &   289 &   295 &   245 \\\bottomrule
\textbf{Total} (TW)&   109 &    90 &    34 &   109 &   102 &    30 \\\bottomrule
\textbf{Down LFR Mean} (MW)&   744 &   802 &   925 &   647 &   744 &   984 \\\midrule
\textbf{Down LFR STD} (MW) &     9 &    16 &    36 &     3 &     9 &    68 \\\midrule
\textbf{Down LFR Min} (MW)&   540 &   268 &  1019 &   720 &   555 &   583 \\\midrule
\textbf{Down LFR Max} (MW)&  1177 &   933 &  1678 &   961 &  1086 &  1424 \\\midrule
\textbf{Down LFR 95 percentile} (MW)&   749 &   791 &  1026 &   718 &   751 &   876 \\\bottomrule
\end{tabular}
\end{center}
\end{footnotesize}

